Making Every Frame Matter: Continuous Activity Recognition in Streaming Video via Adaptive Video Context Modeling

Video activity recognition has become increasingly important in robots and embodied AI. Recognizing continuous video activities poses considerable challenges due to the fast expansion of streaming video, which contains multi-scale and untrimmed activities. We introduce a novel system, CARS, to overcome these issues through adaptive video context modeling. Adaptive video context modeling refers to selectively maintaining activity-related features in temporal and spatial dimensions. CARS has two key designs. The first is an activity spatial feature extraction by eliminating irrelevant visual features while maintaining recognition accuracy. The second is an activity-aware state update introducing dynamic adaptability to better preserve the video context for multi-scale activity recognition. Our CARS runs at speeds $>$30 FPS on typical edge devices and outperforms all baselines by 1.2\% to 79.7\% in accuracy. Moreover, we explore applying CARS to a large video model as a video encoder. Experimental results show that our CARS can result in a 0.46-point enhancement (on a 5-point scale) on the in-distribution video activity dataset, and an improvement ranging from 1.19\% to 4\% on zero-shot video activity datasets.

==> secs/impl.tex <==
% \section{Implementation}



% We implemented our vision encoder CLIP~\cite{radford2021learning} based on the llama.cpp framework~\cite{llama_cpp_impl}, completed the compilation, and carried out INT8 quantization. The existing CLIP.cpp~\cite{clip_cpp_impl} framework based on llama.cpp for compiling CLIP only supports CPU backend, hence it can't utilize the GPU on mobile devices.
% Other mainstream frameworks lack good compatibility for cross-platform deployment.
% For example, OpenClip~\cite{open_clip_impl} and ONNXRuntime-GPU~\cite{onnx_impl} lack support for using the CLIP model with Jetson GPU. 
% We have expanded support for ggml in our implementation, enabling GPU-based inference on all the aforementioned platforms, which resulted in significant system performance improvement. Please refer to Figure~\ref{fig:sys_performance_all}.
% The official implementation of Mamba~\cite{mamba_impl} only supports the PyTorch framework with the CUDA backend. 
% We have compiled our Mamba part into a $C$ program, thereby allowing its deployment on various platforms. 






==> secs/related_works.tex <==
\section{Related Work}
\label{sec:related_works}





\noindent \textbf{Video Foundation Models.}
Recent studies have explored building video foundation models using large language models (LLMs). 
These models achieve impressive results in multiple video understanding tasks~\cite{madan2024foundation}.

Methods like VideoLaVIT~\cite{jin2024video}, VideoLLaVA~\cite{lin2023video}, Video-LLaMA~\cite{zhang2023video}, and Video-LLaMA2~\cite{damonlpsg2024videollama2} use multi-modal pre-training to align visual information with LLMs through projection layers. VideoChatGPT~\cite{maaz2023video} improves video-based conversations by integrating visual encoders with LLMs and instruction tuning. The main challenge in video understanding is handling memory requirements and model capacity, especially for long videos. LaViLa~\cite{zhao2023learning} addresses this by turning LLMs into narrators, allowing them to generate detailed descriptions of long videos from visual inputs. ChatVideo~\cite{wang2023chatvideo} and MM-VID~\cite{lin2023mm} convert videos into text for better comprehension. However, these methods still struggle to model long-range temporal information in streaming videos.


% \subsection{Recent state assistant method for Video Understanding}
\noindent \textbf{Alternatives to Foundation Models for Video Understanding.}
The series of works on Mamba have gained significant attention for overcoming %the local perception limits of convolution and 
the high computational complexity of Transformers as LLMs. 
Recently, Mamba has been applied to various computer vision tasks, showing early progress~\cite{liu2024vision}. However, its application is still in its infancy. 
Mamba-ND~\cite{li2024mambandselectivestatespace} is the first to demonstrate Mamba can handle high-dimensional data and experimentally show the effectiveness in video action recognition. VideoMamba~\cite{li2024videomambastatespacemodel} builds an SSM-based model for video understanding. It shares a similar design with VideoLlama~\cite{damonlpsg2024videollama2} but replaces the Transformer-based LLM with a Mamba-based one for efficiency purposes. 
VideoMamba Suite~\cite{chen2024video} further evaluates Mamba’s performance by integrating it into existing video understanding architectures, showing its potential to handle complex spatial-temporal dynamics.
Unlike these works that use ``all frames at once'' or ``fixed window size'' strategies for Mamba and Transformer video understanding, we propose a lightweight continuous video understanding design with each frame as the input to the state-assistance module.
%Note that, existing works utilize the ``all frames at once'' or ``fixed window size'' strategies, which limits its ability to perform continuous or long video understanding in terms of efficiency and accuracy. 

% Our key insight is to use Mamba for online long-range history modeling by learning the correlations among the dense feature representations of video frames, not just as a replacement for Transformers or Convolutions. 
% We apply this idea to improve video models, significantly increasing the frame rate at which video foundation models can achieve substantial performance gains.
% \qianxi{Do we still need to claim this?}



